Limitations to the energy resolution of single-photon sensitive Microwave Kinetic Inductance Detectors

This paper describes the energy resolution of Microwave Kinetic Inductance Detectors (MKIDs), and models some limiting factors to it. Energy resolution is a measure of the smallest possible difference in energy of the impinging photons, Delta E, that the detector can identify and is of critical importance for many applications. Limits to the energy resolution cause by the Fano effect, amplifier noise, current inhomogeneities, and readout sampling frequency are taken into consideration for this model. This paper describes an approach to combine all of these limitations and predict a wavelength dependency of the upper limit to the resolving power.

==> modelling.tex <==
\chapter{Model and numerical simulation of MKIDs}
\label{modelling}
This chapter describes a study to model two main figures of merit that can describe the performances of an array. The fabrication yield is defined as the number of resonators, expressed as a percentage of the total, with individually-distinguishable resonance frequencies.
This represents the amount of pixels that can be used to reconstruct an image. Two resonators with the same resonance frequency, or with frequencies that are too close to each other, are inherently indistinguishable, therefore it is impossible to trace back which MKID generated the signal.\\
The second parameter of great interest is the energy resolution of each single resonator. The energy resolution describes the smallest possible difference in energy of the impinging photons, $\Delta E$, the detector can identify.\\
A more in-depth description of these figures of merit is given in the next sections along with the description of a model that simulates  the behaviour of MKIDs in order to predict, optimise and design the best array possible.
\section{Fabrication Yield}
 The fabrication of the detectors for such instruments is performed in research-grade clean rooms, through processes which are almost completely human-controlled and not automated. These processes have plenty of room for optimisation, although the fraction of non-responding pixels is less than $1\,\%$. Two or more resonators that resonate at the same frequency while they were not designed for this purpose, are said to be \textit{clashing} or \textit{colliding}. Currently, it is thought that most of the clashes are due to random variations of the critical temperature of the superconductor. Although a systematic radial distribution, over a large area , of critical temperature is known to arise during TiN$_\text{x}$ sputtering deposition \cite{Vissers_2013}, it only plays a negligible role for detectors of chip size is $\approx$ $4$ cm$^2$ as its effect can be dramatically mitigated with an accurate placement of the resonators on the test mask that aims to even out possible drifts in critical temperature and film inhomogeneity .  The current state of the art is that most arrays exhibit a fabrication yield of $75\,\%$ and only for the best ones it goes as high as $80\,\%$ \cite{mazin2020}.\\
The model here discussed is based off the approach described by X. Liu et al in \cite{yield_liu}. 
This simple model relies on a few basic assumptions:
\begin{enumerate}
    \item the array of resonators is infinite on both sides of resonator $\#0$ 
    \item the distance, in frequency space, between two adjacent resonators is designed to be: $f_{n+1} - f_n = \Delta=2$ MHz
    \item the n-th MKID's resonance frequency is randomly distributed about $\Delta n$ according to a gaussian distribution $G(f_n,\sigma)= \frac{1}{\sqrt{2\pi}\sigma} e^\small{{-\frac{1}{2}\left(\frac{(f_n-n\Delta)}{\sigma}\right)^2}}$
    \item given a defined window, a resonator that falls within said window is defined to be clashing. 
\end{enumerate}{}
\begin{figure}
    \centering
    \includegraphics{modelling/model.png}
    \caption{Representation of the simple model of the MKIDs array. Resonances $\# 0$ and $\#\pm1$ are shown as well as the collision window. The probability of two resonators colliding is given by the area underneath the bell curve within the limits of the collision window. }
    \label{model_yield}
\end{figure}{}
The probability that the $0$th resonator does not clash with the nth resonator, P$_{n0}$, can be evaluated, according to \cite{yield_liu}, as one minus the overlapping area defined by the gaussian distribution  and the collision window as described in Figure \ref{model_yield}.
Furthermore, due to the translation symmetry of the model, it is only necessary to evaluate P$_{n0}$ for all values of $\pm n$. The benefit of an infinite array is that allows the following identification:
\begin{equation}
    P_{n0} = 1-  \frac{Erf\left(\frac{n\Delta + \chi w}{\sqrt{2}\sigma}\right) - Erf\left(\frac{n\Delta-\chi w}{\sqrt{2}\sigma}\right)}{2}
\end{equation}{}
Where the integral of a gaussian is evaluated through the error function Erf(x) defined as in Equation \ref{eq:errorfunction}
\begin{equation}
    Erf(x) = \frac{1}{\sqrt{\pi}}\int\limits_{-x}^{+x} e^{-t^2}dt
    \label{eq:errorfunction}
\end{equation}
Here, $\Delta$ is the nominal spacing between the resonators, and  $\chi w$  identifies the collision window through two parameters: $w$ represents the resonator's line-width and a $\chi=5$ is assumed under the hypothesis that the resonators are well distinguishable when separated by $5$ line-widths. This is to say that the profile of the $0$-th resonator is well contained in a window five times larges than its typical line-width. 
Assuming all the resonators to be independent, the total yield is derived as:
\begin{equation}
    Yield = \prod\limits_{n= -n_{max}}^{n_{max}} P_{n0}
    \label{eq:yield}
\end{equation}{}
\noindent
For the sake of a model, it was assumed  that  the MKID $\#0$ resonates at the central frequency of the working bandwidth, $6$ GHz. And only the first $1000$ resonators left and right have been taken into consideration. The identification \ref{eq:yield} is only valid in the case of an infinite array of evenly spaced resonators.
The analysis of this model will be carried out in the next few pages and the dependencies of the yield from physical parameters such as the quality factor of the resonators and the critical temperature of the superconductor will be investigated. It is possible to observe that while increasing the spacing $\Delta$ between two consecutive elements of the array, the yield increases accordingly.\\
\vspace{0.5cm}
A question left unanswered, this far, is how the frequency of an ideal resonator changes when the desired T$_c$ is not met. 
A simple approach follows the discussion described in \cite{Annunziata} and \cite{Tinkham}; the dependence of the kinetic inductance as a function of the temperature can be evaluated as:
\begin{equation}
    L_{k}=\frac {l}{w}\frac {R_{s}h}{2\pi ^{2} 1.76 T_{c_0} }\tanh \left( \frac {1.76 T_{c_0} }{K_{B}T}\right)
\end{equation}{}
Where $R_{s}$ is the resistivity of the film in its normal state, l and w are the physical length and width of the film, h is its thickness, $T_{c0}$ is the critical temperature of the film and $k_B$ is Boltzmann's constant.\\
Given the change in kinetic inductance, and knowing that the resonance frequency of an LC circuit $f_r = \frac{1}{\sqrt{LC}} $ the fractional frequency shift in resonance frequency induced by a change in critical temperature, therefore a local change in kinetic inductance, is easily obtained  provided three  assumptions are met : 
\begin{enumerate}
    \item The capacitance of the resonator is only due to its geometry
    \item The inductance is only due to the kinetic inductance. The kinetic inductance fraction $\alpha = 1$
    \item Any change in sheet resistivity R$_s$ with T$_c$ is negligible.
\end{enumerate}{}
Under these circumstances, the fractional frequency shift is given by Equation \ref{eq:freq_shift1}\\
\begin{equation}
\label{eq:freq_shift1}
\frac{\Delta f}{f_r}(Tc)= \frac{\frac{1}{\sqrt{L(T_c)C}}- \frac{1}{\sqrt{L(T_{c_0})C}}}{\frac{1}{\sqrt{L(T_{c_0})C}}}
\end{equation}
Here the previous assumptions take a critical part, as $L(T_c)= L_K(Tc) + L_g$ where the latter term represents the geometric inductance.The hypothesis that $\alpha\approx1$ allows to neglect $L_g$ with respect to $L_K$ and the assumption that $R_s$ does not change with stoichiometry allows to simplify Equation \ref{eq:freq_shift1} as:
\begin{equation}
    \frac{\Delta f}{f_r}(Tc)= \frac{\sqrt{\frac{1}{T_c}\frac{1}{\tanh{\left(\frac{1.76 T_{c_0}}{2k_BT}\right)}}}^{-1} -\sqrt{\frac{1}{T_c_0}\frac{1}{\tanh{\left(\frac{1.76 T_{c_0}}{2k_BT}\right)}}}^{-1}}{\sqrt{\frac{1}{T_c_0}\frac{1}{\tanh{\left(\frac{1.76 T_{c_0}}{2k_BT}\right)}}}^{-1}} 
    \label{eq:freq_shift2}
\end{equation}{}
Where $\Delta f = f_r(Tc) - f_r(T_{c_0}), $ T$_c_0$is the desired critical temperature, $800$ mK for the sake of this discussion; T is the equilibrium temperature at which the MKIDs array is operated, $100$ mK. Figure \ref{Tc_freq} shows the absolute value of Equation \ref{eq:freq_shift2} as a function of the temperature difference $T_c - T_{c0}$.\\
The main purpose of this calculation is to try and estimate reasonable boundaries for the width $\sigma$ of the distribution of the frequencies about their mean value $f_n$. Although, Equation \ref{eq:freq_shift1} is asymmetrical around T$_{c0}$ , for small $T_c$ variations, the two branches can be considered symmetrical as a fist order approximation. It is assumed that only $0.1\%$ of the resonators have a critical temperature that differs by more than $200$ mK, thus a shift in resonance frequency that is greater than $1.2$ GHz. This justifies the assumption of an upper limit for $\sigma = 0.300$ GHz. Such a broad distribution would be catastrophic for any real array and is certainly overestimate of any realistic value of $\sigma$ in any well-behaved array .\\
\begin{figure}[h!]
\begin{minipage}[b]{0.5\textwidth}
    \includegraphics[width=\textwidth]{modelling/Fig2.png}
\end{minipage}
\begin{minipage}[b]{0.5\textwidth}
  \includegraphics[width=\textwidth]{modelling/Figure33.png}
\end{minipage}
  \caption{Left: fractional frequency shift as a function of critical temperature fluctuations. Right: yield as a function of $\sigma$, evaluated  for a collision window of $0.5$ MHz. The inset shows a wider span of values of $\sigma$, up to $0.6$ GHz.}
  \label{Tc_freq} 
\end{figure}{}


%\begin{figure}[h!]
%    \centering
%    \includegraphics[scale=0.6]{modelling/Tc_freq.png}
%    \caption{}
%    \label{Tc_freq}
%\end{figure}{}
A first evaluation of the fabrication yield is carried out to understand how well this simple model describes the collective behaviour of an array of MKIDs. A particular choice of the free-parameters is made; it is worthwhile describing the fabrication yield as a function of a varying $\sigma$ in order to justify how big an effect our previous assumptions have, and instead of evaluating the line-width of the resonators, the current working assumption is that the total width of the collision window is $ 0.5$ MHz.\\

Figure \ref{Tc_freq} (Right) shows the yield starting to roll off as soon as the standard deviation of the distribution of the resonance frequency around its centre value is comparable to the spacing between two adjacent resonators $\Delta_r$. The yield eventually flattens for values of $\sigma \ge 0.2 $ GHz at about $75\%$. Unfortunately, due to its inherent limitations, it is quite difficult to compare the results produced by the model with experimental results. Nonetheless, it is important to also include in the dissertation how the total quality factor $Q_{tot}$ of the resonators comes into play in this model. By definition, the higher the quality factor $Q$, the sharper is the resonator's dips Q is inversely proportional to the line-width $w = \frac{f_0}{Q}$ where $f_0$ is the characteristic resonant frequency. Assuming a $\Delta_r= 2$ MHz, and based on formula \ref{eq:yield}, Figure \ref{yield} shows a 2D plot of the fabrication yield as a function of both  $\sigma$ and $Q$. Two trends are visible in the plot. The yield increases with increasing quality; this says that the sharper the resonator, hence the smaller their line-width and the clashing window, the higher the fabrication yield is. Also, as expected, the smaller the width of the  frequency scatter distribution, the higher the yield per fixed values of $Q$. \\
Very strongly coupled resonators with low quality factors, such as $Q_{tot}< 15000$, represent the case where the resonator's rejection window is intrinsically larger than the spacing $\Delta_r$ reducing dramatically the yield to a mathematical zero based on previous assumptions. For very high values of $\sigma$, the model is, in fact, describing an almost random distribution of resonant frequencies. It therefore makes sense that the yield becomes proportional to the rejection window size, thus to the total quality factor $Q_{tot}$.

\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{modelling/YIELD_25032020.png}
    \caption{Fabrication yield as a function of the overall quality factor $Q$ and the width of the frequency scatter distribution, $\sigma$.}
    \label{yield}
\end{figure}{}
It is crucial to state the flaws and the limits of this model and discuss the possible improvements of said picture. There are two main issues to discuss: first of all, a gargantuan value of $\sigma$ would produce a $100\%$ yield as it would scatter most of the resonators outside the working-bandwidth,$4-8$ GHz. It was observed that the yield starts increasing from $\sigma = 1$ GHz onward. Another limit of the model is that, when evaluating the probability of a collision, only one of the two resonator's dips is broadened, while the other is still regarded as if it was infinitely sharp. This effect is only relevant for very strongly coupled resonators, $Q_{tot} > \frac{1}{\sigma}$, therefore it is not  significant for the plot in  Figure \ref{yield}. Further improvement, which is a higher-order approximation to what has been discussed so far resides in the evaluation of the line-width as a function of the specific resonator's resonance frequency. 
In order to summarise the results described in the previous pages, Table \ref{tab:yield} represents some numerical results for interesting parameters.\\
\vspace{0.5cm}
\begin{table}[h!]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
    \sigma\, (MHz)  & Q_{tot} & Yield\,(\%)  \\
    \hline
    
    0.8 & 20000 &79.8\\
    \hline
    0.6 & 20000 & 89.9\\
    \hline
    1.8 & 30000 & 73.8\\
    \hline
    1.4 & 30000 & 85.5\\
    \hline
    1.0 & 30000 & 95.7\\
    \hline
    2.4 & 50000 & 75.8\\
    \hline
    1.8 & 50000 & 87.8\\
    \hline
    1.4 & 50000 & 95.3\\
    \hline
    4.2 & 100000 & 74.4\\
    \hline
    2.8 & 100000 & 84.0\\
    \hline
    1.8 & 100000 & 94.8\\
    \hline
    \end{tabular}
    \caption{Table representing the yield of a 2000  pixel array as a function of $\sigma$ and the total quality factor $Q_{tot}$}
    \label{tab:yield}
\end{table}{}

\section{Resolving Power}
For detectors, such as MKIDs, that can measure the energy of the incident radiation, energy resolution is a critical figure of merit. The best way to describe it is, borrowing Dr. W. R. Leo's words,  " [...] the extent to which a detector can distinguish two close lying energies" \cite{WRLeo}. 
An ideal detector,   when illuminated by monochromatic light would produce a spectrum that is also monochromatic, and hence described by a Dirac's $\delta$ function.  In reality, the width of the spectral lines is finite, broadened by several factors which lead to what is experimentally observed. For the sake of clarity, the energy resolution of a detector is intended as $\frac{\Delta E}{E}$, The quantity that will be evaluated most of the time is its inverse  $\frac{E}{\Delta E}$ is referred to as the  Resolving Power. 
At present, deVisser et al. \cite{deVissersphononiccrystal} claim that the best resolving power achieved corresponds to  $\frac{E}{\Delta E} \sim 55$ for wavelengths between $402-1545$ nm. The next few page will describe how the following effects come into play in broadening  the spectral peak: \\
\begin{enumerate}
    \item Statistical processes in the MKID
    \item Amplifier noise - High Electron Mobility Transistor
    \item Current density inhomogeneity
    \item Readout frequency
    \item Two-level systems 
\end{enumerate}{}
\subsection{Energetic processes in the MKID}
As stated in \cite{Guo}, the best energy resolution an MKID can achieve as a pair-breaking detector is given by $R = \frac{\Delta E}{E} = {2.355}\sqrt{\frac{F\Delta_s}{\eta h\nu}}$, where $\eta\approx 0.57$ is the pair-breaking efficiency \cite{EnergyDownconversion}, $h\nu$ is the energy of the impinging photon, $\Delta_s = 1.72 k_B T_c$ is the superconducting gap energy of the adsorbing material. $F$ is the Fano factor, the effect of which encompasses all the statistical processes that do not lead to pair-breaking. A typical value of the Fano factor  for superconductors is $F=0.2$. These parameters yield a maximum energy resolution of $0.011$ for $\lambda_0 = 650$ nm. Unfortunately, there is little room for improvement. For other kind of energy resolving detectors, such as gas and silicon based ionisation detectors, the Fano factor  is known to vary, quite significantly, with the material according to \citet{Fano_material,fano_gas1}. The Fano factor is an inherent property of the material and perhaps it is worth investigating whether different superconductors exhibit different Fano factors. the pair-breaking efficiency, which compares the average number of quasiparticles produced per photon with the maximum number of quasiparticles  that can be produced, can be marginally improved by changing the design of the resonator \cite{pairbreakingefficiency}. Studies carried out in SRON by deVisser et al. \cite{deVissersphononiccrystal} suggest that hot-phonon loss accounts for some of the losses. In particular, hot-phonon loss contributes to increasing the Fano factor by a factor $J$.
\begin{equation}
R = \frac{\Delta E}{E} = {2.355}\sqrt{\frac{(F+J)\Delta_s}{\eta h\nu}}
\end{equation}
An analytical model and experimental measurements demonstrated that for both Si and SiN substrates, $J\approx 3$, whereas it is higher for Sapphire substrates. The same paper \cite{deVissersphononiccrystal} proposed the implementation of MKIDs where the inductors are fabricated on a membrane so to reduce phonon losses. This should reduce the energy loss through phonon mediated processes to the silicon substrate, effectively eliminating phonon loss and thus maximising the pair breaking efficiency. Unfortunately, a value of $\eta = 1$ cannot be achieved since any photon of energy greater than $2\Delta$ but smaller than $4\Delta$ will only create $2$ quasi particles and phonon excitations that can not break up any further amount of Cooper Pairs. For higher energies, the efficiency depends on phonon trapping factor \cite{pairbreakingefficiency}where improvement is possible.
\subsection{High Electron Mobility Transistor noise}
\label{sec:HEMT}
High Electron Mobility Transistors are likely one of the main limiting factors when it comes to Energy Resolution. The HEMT discussed here is the Low Noise Factory LNF-LNC4$\_$8C which is a ultra-low noise cryogenic amplifier operating in the $4$-$8$ GHz bandwidth. Its nominal noise temperature, as stated by the manufacturer, is  $2.1$ K.\\
The HEMT random noise affects the phase signal. In particular, when a photon strikes the MKID, the phase signal generated is added to this noise and, of course, the height of the phase-jump has an uncertainty given by the noise contribution of the HEMT itself. Referencing Figure \ref{fig:model_hemt}, the quantity that has to be evaluated is $\mathcal{R} = \frac{\Delta\alpha }{\alpha}$. Assuming that the MKID taken into consideration is optimised to respond with an $\alpha = \pi$ phase shift when struck by a  photon of wavelength $\lambda_0 = 650$ nm. Figure \ref{fig:model_hemt} shows the angles just discussed and is of critical importance for the understanding of the model.\\
\begin{figure}[h!]
    \centering
    \includegraphics{modelling/model_hemt.png}
    \caption{Schematic of a resonance loop. The large circle describes the cable delay, the smaller circle is that characteristic of a resonator. Two angles are highlighted: $\pi$ and $\Delta \alpha$. The latter describes random phase fluctuations due to the HEMT noise. For the sake of clarity, the centre of the IQ plane was shifted away from the centre of the loop.}
    \label{fig:model_hemt}
\end{figure}{}
HEMT noise induces random fluctuations in both I and Q. Therefore, a non illuminated MKID produces a signal in the I-Q plane that is represented as a scattered cloud. When a photon is detected, the cloud is added to the photon induced phase signal generating inaccuracy regarding the photon's phase signal $\Delta \alpha$ .
To clarify, the quantity to evaluate is $\Delta \alpha$, the angle defined by the radius of the resonant loop and the amplitude of the phase noise. In particular, it is not trivial to understand how the noise temperature of the amplifier is then translated into phase noise.\\
Jonas Zmuidzinas' 2012 review \cite{Zmuidzinas} helps; assuming that the amplifier noise is equally distributed between the $I$ and the $Q$ component the noise component can be described by the following equation: 
\begin{equation}
 HEMT\_noise = \sqrt{\frac{k_B T_A G}{2P_{MKID}} BW}
\label{eq:noise-hemt}
\end{equation}{}
A thorough derivation of the equation is given in the Appendix \ref{appendix:HEMTnoise}
where $k_B$ is Boltzmann's constant, T$_A$ is the noise temperature of the amplifier, $G$ is the gain of the amplifier, $P_{MKID}$ is the power at the HEMT and $BW$ is the bandwidth given by the Fast Fourier Transform sampling rate, $1$ MHz.  Equation \ref{eq:noise-hemt} describes both the I and Q components of the HEMT noise in I and Q units. Now, geometrical considerations, based on maximum and minimum transmission (S$_{21}$), lead to a simple formula for $\Delta \alpha $
\begin{equation}
    \Delta \alpha = \frac{HEMT\_noise}{radius}
\end{equation}{}
Where $HEMT_{noise}$ is the length of the arc described by the cloud, and $radius$ is the radius of the resonant loop. Assuming perfect transmission in the cable delay loop,  which is described by a circle of unit radius. Knowing the distance from the origin of the resonance frequency of a non illuminated MKID is $min |S_{21}|$, and by definition of  $Q_c$ \cite{Zmuidzinas},  $Q_C = \frac{Q}{1- min|S_{21}|} $ , it is possible to obtain
\begin{equation}
    \Delta \alpha = 6 \frac{HEMT\_noise\,\, Q_c}{Q}
\end{equation}{}
Where $Q_c$ is the coupling quality factor, $Q$ is the total quality factor of the MKID. The  value of $\Delta \alpha$ would only describe the rms of said quantity. There is  an additional factor of $3$ to account for the conversion from a rms quantity to a peak-to-peak quantity.\\
\begin{figure}[ht!]
\includegraphics[scale=0.25]{modelling/HEMTNOISE_Power.png}
  \label{fig:HEMT_power} 
  \caption{HEMT noise, $\frac{\Delta\alpha}{\alpha}$ as a function of the power at the resonator. Standard operating powers are in the $-100$dB range.}
\end{figure}{}
While it may seem that the noise component is very low, it is important to observe that usual readout power, before entering the cryostat, would be $\approx-50 $ dBm, in addition to that, two $20 $ dB attenuators have to be taken into account as well as the attenuation of the coaxial cables going into the cryostat. Assuming a total power at the HEMT of about $-90 $dBm, $Q_i= 100000$ and $Q_c=45000$,  $\frac{\Delta\alpha}{\alpha} \approx 0.037$. It corresponds to a noise fluctuation of $\pm 3.3^\circ$  in good agreement with common measurements of  $\pm5 ^\circ$ white noise in baseline.  
\begin{figure}[h!]
    \includegraphics[scale= 0.3]{modelling/HEMTNOISE_mammeta.png}
    \caption{2D graph showing the dependency of the HEMT noise  in degrees, assuming that a photon produces a $180^\circ$ signal, as a function of the coupling quality factor $Q_c$ and the internal quality factor $Q_i$. It is important to observe that the area shaded in yellow,represents the parameter space where the HEMT noise is  equal o  greater than $36^\circ$. }
    \label{fig:HEMT_QQ}
\end{figure}{}
As a final remark, figure \ref{fig:HEMT_QQ} shows a 2D plot which clarifies the dependence of $\Delta\alpha/\alpha$ on both the internal quality factor $Q_i$ and the coupling quality factor $Q_c$. The plot here shown refers to a power value $P_g = -90$ dBm. The area shaded in yellow depicts a portion of the parameter space where $\Delta \alpha / \alpha \ge 0.2$, or $\pm36^\circ$.
\subsection{Current density inhomogeneity}
Another source of uncertainty in the response of an MKID is inhomogeneity of the current density across the inductor. If the current density varies spatially across the inductor, the resulting signal from an absorbed photon will depend on absorption location as  variations in current density lead to  changes in responsivity $d\theta /dN_{qp}$; where $\theta$ is the phase angle, the measured response of the MKID to a photon strike, and $N_{qp}$ is the number of quasi-particles produced by the photon. Current density uniformity strongly depends on the resonator's geometry. Current crowding at right angles is a well known effect for both normal metals and superconductors \cite{current-crowding}. The current density is affected by the capacitance of the interdigitated capacitor. The charge carriers tend to slow down and create high electric field as they drift towards the two plates of the capacitor resulting in a small, but non negligible gradient in current. The current density is highest at the top of the inductor (far from the capacitor) and sees a typical $5\%$ reduction in proximity of the capacitor. This is because the change in density of the super current induced by a photon depends non-linearly on the intensity of the current. This reflects its effect on both the shift in resonance frequency and the total quality factor $Q_{tot}$. The change in $Q_{tot}$ accounts for an internal change in $Q_c$ which depends on the resonant frequency of the resonator, while a more significant change in $Q_i$ can be attributed to losses through  normal-state electrons produced by pair breaking.  In order to evaluate the effects of current density inhomogeneities, the current density data, simulated with SONNET with a grid size in both $x$ and $y$ direction of $0.125\,\mu$m  (Figure \ref{fig: map1}) is imported to a Python script I developed.The data is read in by the programme and it is then normalised to the average value over the whole inductor.  This creates a current density map which is, for the most part, in the range [$0$,$1$] with values greater than $1$ only in the inner part of right-corners, where there is a significant current crowding. The working assumption for the next steps is that each single element of the inductor, as defined by the simulation through the grid size, contributes to the total kinetic inductance of the resonator with its elemental contribution and the total kinetic inductance is given by the the sum of the contributions of all the single elements. The resonator is designed in such a way that its resonant frequency is $f_0 = 6$ GHz and $Q_c = 30000$.  \\
\begin{figure}[h!]
\begin{minipage}[b]{0.49\textwidth}
    \includegraphics[scale=0.2]{modelling/Figure_1.png}
\end{minipage}
\begin{minipage}[b]{0.49\textwidth}
  \includegraphics[scale=0.2]{modelling/Figure_6.png}
\end{minipage}
  \caption{Left: Current density map of the inductor. Right: Phase shift when struck by a photon as a function of the ($x$,$y$) position.}
  \label{fig: map1} 
\end{figure}{}
The Python programme, was fed the current density data produced by SONNET, translates the current density 2D-map first into a Kinetic Inductance 2D-map, by knowing the inductance depends on the current density at the location of each of the cells. Once the kinetic inductance of the whole circuit is known, its resonant frequency is immediately given by $\tfrac{1}{\sqrt{L_K C}}$.
When a photon strikes on a specific point of the inductor, it depletes the region around it of charge carrying Cooper Pairs increasing  the kinetic inductance of the resonator. As a consequence of this increase of kinetic inductance, the aforementioned shift in resonance frequency , and phase, occurs. Figure \ref{fig: map1} (Left) shows the expected resonance frequency shift according to where the photon strikes on the inductor. Here, for the sake of simplicity the diffusion of the quasi-particles in the superconductor was not taken into account. \\ It is possible to evaluate the phase shift registered at the readout frequency, $6$ GHz for the sake of this simulation, and it can be iterated for all the possible grid elements produced by SONNET. Manipulating equation \ref{eq:s21} to obtain the  phase  component, it is possible to produce the 2D map shown in Figure \ref{fig: map1} (Right) where it is shown the phase shift, measured at $f_0 =6$ GHz, due to an impinging photon as a function of the position where the photon hits the inductor. In order to simulate a well optimised resonator at the impinging wavelength, the depletion considered was that which produces a $\geq 0.95\,\pi$ phase shift. \\
\begin{figure}[h!]
\centering
    \includegraphics[scale=0.6]{modelling/profile1.png}

  \caption{Histogram of Figure \ref{fig: map1}. Where $\alpha$ is $\approx 0.965\,\pi $ radians. The designed resonant frequency, in dark, is $6$ GHz and the total quality factor is $Q_{tot} = 30000$. }
  \label{fig: map2} 
\end{figure}{}
As previously discussed in Section \ref{sec:HEMT}, the Energy Resolution $R=\frac{\Delta E}{E}$, can be described in terms of $\frac{\Delta \alpha}{\alpha}$. Figure $\ref{fig: map2}$ (Left) represents the frequency histogram of the phase values in Figure \ref{fig: map1} (Right). The full width of the profile represents $\Delta \alpha$, whereas the peak value is representative for $\alpha$.  Under these circumstances and, based on these assumptions, for $f_0 = 6$ GHz and $Q_{tot} = 30000$, $\frac{\Delta \alpha}{\alpha} = 0.004$.



As a final remark, it is interesting to evaluate if and how $\frac{\Delta \alpha}{\alpha}$ depends on the total quality factor $Q_{tot}$. A plot of such dependence is shown in Figure \ref{DA_q}. This model hints that a small improvement can be obtained by  increasing the resonator's total quality factor.\\
In reality, the model does not include the effects of dissipative effects induced by the excited quasi-particles, which behave like normal-state electrons. These losses account for a reduction in the internal quality factor $Q_i$ and have not been included in the discussion. 
\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.35]{modelling/Da_a vs Q.png}
    \caption{Dependence of $\frac{\Delta \alpha}{\alpha}$ as a function of $Q$}
    \label{DA_q}
\end{figure}{}

\subsection{Sampling frequency}
The last effect that is taken into consideration is the interplay between the sampling rate of the ADCs, that also affects the amplification noise, see Section \ref{sec:HEMT} in the readout electronics, and the  quasi-particle lifetime. The \textit{cardinal theorem of interpolation}, as formulated by Nyquist  \cite{Nyquist} and Shannon \cite{Shannon}, describes a classical problem in sampling. When the ADC digitises the analogue signal at its input, it creates a form of uncertainty in the maximum of the phase signal. According to the aforementioned theorem, during sampling, the frequencies higher than half of the sampling frequency, cannot be properly sampled and reconstructed, therefore both the rising  and the trailing edge of the phase signal are subject to uncertainties. It is impossible to identify with absolute certainty where the peak lays and what its real value is. The ADC  used on ROACH boards is commonly operated with a  $1$ MHz sampling rate, therefore, it is possible to constrain the location of the maximum within a $1\,\mu$s time frame. In particular, $1\,\mu$s is enough time to take account of the ring-down time of the resonator. Given this uncertainty, and knowing the quasi-particle recombination time, it is easy to evaluate how a $1\,\mu$s interval is reflected  into an error on the phase value. A schematic picture is shown in Figure \ref{ADC_freq}. The recombination time for this model is $100\,\mu$s; which is a typical value for TiN$_x$ resonators. 
\begin{figure}[h!]
    \centering
    \includegraphics{modelling/sampling.png}
    \caption{The uncertainty on phase angle depends on the sampling rate and the quasi-particle recombination time.}
    \label{ADC_freq}
\end{figure}{}
\begin{equation}
    \frac{\Delta \alpha }{\alpha } =1-e^{-\frac {\Delta t}{\tau _{qp}}}
\end{equation}{}
Where $\Delta t$ is the time interval between two points being sampled and $\tau_{qp}$ is the quasi-particle recombination time. For a sampling rate of $1$ MHz and a recombination time of $100\,\mu$s, \\
\begin{equation}
    \frac{\Delta \alpha }{\alpha }= 0.00995
\end{equation}{}
Obviously, a faster sampling rate coupled to a faster FFT would help, as one order of magnitude alone would result in an improvement in $\frac{\Delta \alpha}{\alpha}$ from $\sim 0.01$ to $\sim 0.001$. The other option, would require the use of a superconducting layer with an intrinsic recombination time that is longer than $100\,\mu$s. Although this is possible in theory, depending on the application, it may not be possible for practical reasons as a longer recombination time would imply a longer \textit{dead time} of the detector. 
\subsection{Two-Level System Noise}
MKIDs exhibit an "excess" phase noise that is not fully described by the components previously discussed which is commonly referred as two-level systems (TLS) noise. The internal quality factor $Q_i$ of a resonator is often limited not by the losses internal to the superconductor, rather by dissipation through TLS. TLS noise is primarily due to the coupling of the electric dipole moment of two-level systems with the electric field of the resonator. In particular, since the interdigitated capacitors tend, by their own nature, to sustain high electric fields the capacitors are considered  the TLS-noise producing element of an MKID. Even though a semi-empirical model for TLS noise has been developed, I will not delve into it. Instead it is interesting to evaluate the contribution to the phase noise solely due to TLS. \\
When probing  MKIDs arrays with tones at -$90$ dBm,  a typical phase noise of $\pm 5^\circ$ has been observed. According to the calculations carried out in the previous section, one might assume the HEMT phase noise of $\pm 3.3^\circ$; with the remainder, $\pm 1.7^\circ$ can be addressed as TLS noise. TLS noise is well known to saturate as the power of the probe tones increases resulting in an increase in the signal to noise ratio. The description of this behaviour is beyond the scope of this work and will not be discussed. Instead, Table \ref{tab:TLS}, shows the value of $\frac{\Delta\alpha}{\alpha}$ for different values of the noise component due to TLS.
\begin{table}[h!]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline
    TLS noise & $\pm 0.5^\circ$  & $\pm 0.7^\circ$ & $\pm 2.5^\circ$ & $\pm 10^\circ$ \\
    \hline
    $\frac{\Delta \alpha }{\alpha}$& 0.0056& 0.0189  & 0.0278 &  0.111 \\
    \hline
    \end{tabular}
    \caption{Contributions to $\frac{\Delta \alpha}{\alpha}$ for different values of TLS phase noise, in degrees.}
    \label{tab:TLS}
\end{table}{}

\subsection{Energy resolution}
The connection between the energy resolution $R =\frac{\Delta E}{E}$ and the parameter here discussed $\frac{\Delta \alpha}{\alpha}$ still has to be established. First of all, a cumulative value for $\frac{\Delta \alpha}{\alpha}$ can be obtained on the hypothesis that the four contributions are independent and their quadratures can be added up to an overall distribution width.
\begin{equation}
    \frac{\Delta \alpha}{\alpha} = \sqrt{\left(\frac{\Delta \alpha }{\alpha}\right)_{HEMT}^2 + \left(\frac{\Delta \alpha} {\alpha}\right)_{Currents}^2+\left(\frac{\Delta \alpha}{\alpha}\right) _{Readout}^2+\left(\frac{\Delta \alpha}{\alpha}\right) _{TLS}^2} = 0.0429
\label{eq:DAA_00249}
\end{equation}{}
Where the HEMT noise accounts for the most part, and the contribution due to the current inhomogeneity is about an order of magnitude smaller than that of the HEMT. The three quantities are represented in Table \ref{tab:daa}.\\
\begin{table}[h!]
    \centering
    \begin{tabular}{|c|c|c|c|}
    \hline
    $\left(\frac{\Delta \alpha }{\alpha}\right)_{HEMT}$ & $\left(\frac{\Delta \alpha }{\alpha}\right)_{Currents}$ & $\left(\frac{\Delta \alpha }{\alpha}\right)_{Readout} &  $\left(\frac{\Delta \alpha }{\alpha}\right)_{TLS}$ $\\
    \hline
    0.037 & 0.004 & 0.0095 &0.0189\\
    \hline
    \end{tabular}
    \caption{Typical contributions to $\frac{\Delta \alpha}{\alpha}$ from the main sources of noise: HEMT, Current inhomogeneity, Readout frequency and TLS.}
    \label{tab:daa}
\end{table}{}
Even though it is intuitive that $\frac{\Delta \alpha}{\alpha}$ and $R = \frac{\Delta E}{E}$ are related, it is not straightforward to compare $R_{Fano} = 0.01116$ and $\frac{\Delta \alpha}{\alpha} = 0.0385$. While deriving an analytic function that describes the angular displacement in the IQ plane as a function of the photon energy is possible, and an attempt is described in Appendix \ref{appendix:eq-DeltaE}, it is perhaps not the optimal choice for the sake of this work.
A more practical approach when working with detectors is to use a number of calibration wavelengths. By illuminating the detector with monochromatic light of selected wavelengths ($\lambda_i...\lambda_n)$ and based on the response of the detector at each wavelength, it is possible to trace a calibration curve. Often times, this curve is simply given by a linear interpolation between every two adjacent calibration points. In each segment of the calibration curve the identification described by Equation \ref{eq:daa_2} is correct:\\
\begin{equation}
    \frac{\Delta E}{E} = \frac{\Delta \alpha}{\alpha} 
\label{eq:daa_2}
\end{equation}{}
The only assumption that is necessary to explicit is that at every wavelength the width of the angular distribution $\Delta \alpha$ caused by a a photon of wavelength $\lambda$ is either confined within the individual segment defined by $\lambda_j < lambda \lambda_{j+1}$ or on its extrapolation. Based on these assumptions, the energy resolution corresponding to a value of $\frac{\Delta \alpha}{\alpha} = 0.0429$ is $R_{\alpha} = 0.0752$. The two contributions to the energy resolution can now be added in quadrature:
\begin{equation}
    R = \sqrt{R_{Fano}^2 + R_{\alpha}^2} = 0.0748
    \label{eq:ENRES}
\end{equation}{}
This means that when illuminated by a red photon, $\lambda = 650$ nm, the wavelength used as an example  for the entire length of this chapter, the MKID taken into consideration will detect its energy to be $1.907\pm 0.142 $ eV corresponding to a resolving power, $P= \frac{E}{\Delta E} = 11.52$.\\
It is worth taking a moment to break down the different contributions that limit the detector's performance. In order to do so, it is possible to individually neglect the elements in Equations \ref{eq:DAA_00249} and \ref{eq:ENRES} and then list them from the most to the least detrimental: The noise component that limits  the performance of the detector the most is that induced by the HEMT. If one could, ideally, reduce it to zero, the resolving power would increase to $P=17.35$. The second element that contributes is given by hot-phonon losses. If one could reduce phonon losses to a negligible amount, the resolving power would increase to $25.75$. Then comes two level systems (TLS) noise, neglecting which, would bring the resolving power up to $P=47.24$. The readout electronics reduces the resolving power from $P=76.65$  and finally  the contributions given by the Fano noise     and current inhomogeneities, which, when the contribution due to all the other noise sources have been neglected, alone limit the resolving power to $P=142.50$.   
One final comment is on the wavelength dependencies of some the main contributors to the energy resolution limits. In particular, it is immediate that the readout sampling frequency has no dependence on the wavelength at which the resonator is being illuminated. It is intuitive that the current inhomogeneity is present in the superconducting inductor independently on the impinging photon's wavelength. Obviously, a resonator optimised to produce a $180^\circ$ phase shift for $650$ nm will produce a smaller signal when detecting less energetic photons, and the ratio $\frac{\Delta \alpha}{\alpha}$ due to it is dependent on the wavelength.\\
Things get more complicated when considering the effects of the HEMT, and its noise temperature, on the signal. In this case, $\Delta \alpha$ can be assumed to remain constant independently on the wavelength on the impinging photon, whereas the absolute value of $\alpha$ changes with wavelength, effectively decreasing the signal to noise ratio, and thus reducing the energy resolution of the detector. Furthermore, this case is not easy to discuss as the identification in Equation \ref{eq:daa_1} and Equation \ref{eq:daa_2} are not valid anymore. Under this circumstance it is not correct to claim that $E_{max}$ describes the value of $E$ if the resonator produces a phase response that is significantly different from $\pi$ radians.\\
Finally, the Fano contribution deserves some attention as it may have gone unstated that the value of $R_{Fano}$ is wavelength dependent, and it is ranges from $\approx 0.075$ for highly energetic blue photons ($300$ nm) to $\approx 0.017$ for infrared photons ($1500$ nm). 
\subsection{Energy dependence}
Following the arguments discussed in the previous section, it is established that the Energy Resolution is wavelength dependent, therefore the empirical evaluation of said dependency could be of great interest. Investigating in detail the effect requires great effort, moreover, interlinking the several physical processes that contribute to the description of the effect is not easy. An easier approach is to imagine a resonator of which the response is above the noise level over the whole range of wavelengths of interest: from $650$  to $1650$ nm. Ideally, the resonator would be optimised to produce a $180^\circ$ phase signal when struck by a $650$ nm  photon and would produce a signal which is still discernible from the noise at $1650$ nm, let us assume one order of magnitude above the noise threshold, e.g. a $50^\circ$ phase shift. Ideally, one could imagine the phase shift produced by the resonator to be directly dependent on the wavelength of the impinging photon. Under these assumptions, the height of the phase pulse would be described by Equation \ref{eq:phase-linear}
\begin{equation}
    \alpha = 180 - 0.13(\lambda - 650)
\label{eq:phase-linear}
\end{equation}
The different components that make up $\frac{\Delta \alpha}{\alpha}$ might or might not dependent on the value of $\alpha$: the contributions due to current crowding and inhomogeneity, TLS noise, and the HEMT noise depend on the pulse height. Given the same amount of noise produced by the resonator or the HEMT will have a different impact on the detector's performance depending on the height of the phase pulse. On the contrary, given the self-similarity of the exponential decay, the contribution due to the readout electronics and its sampling frequency does not depend on the height of the signal. Under these assumptions, Equation \ref{eq:DAA_00249} becomes:
\begin{equation}
    \frac{\Delta \alpha}{\alpha}\left(\lambda\right) = \sqrt{\left(\frac{\Delta \alpha }{\alpha}\left(\lambda\right)\right)_{HEMT}^2 + \left(\frac{\Delta \alpha} {\alpha}\left(\lambda\right)\right)_{Currents}^2+\left(\frac{\Delta \alpha}{\alpha}\left(\lambda\right)\right) _{TLS}^2+\left(\frac{\Delta \alpha}{\alpha}\right) _{Readout}^2} 
\label{eq:DAA-lambda}
\end{equation}{}
where the $\lambda$ dependency of the parameter $\alpha$ is described by Equation \ref{eq:phase-linear}. The curve described by Equation \ref{eq:DAA-lambda} is shown in Figure \ref{fig:DAA-lambda}. The equation that links $\frac{\Delta \alpha}{\alpha}$ to the energy resolution $\frac{\Delta E}{E}$ is only accurate when the resonators are well optimised for the specific wavelength, which means, when the phase pulse it produces is $\approx 180^\circ$. Keeping in mind that this identification is only exact for wavelengths close to $650$ nm, it is possible to extend it over the whole wavelength range of interest in order to gather qualitative information about the trending of the curve, which is shown in Figure \ref{fig:DAA-lambda}. The scatter plot shows resolving power values measured by different groups for MKIDs made of different materials: Guo et al., \cite{Guo},  (Green)  for their TiN/Ti/TiN MKIDs measured a value of  $P =3.7$ at $1550$ nm, in agreement with what predicted by the model $P=3.77$, Szypryt et al., \cite{Szypryt_2017}, (Red) obtained a resolving power in the wavelength range $808- 1310$ nm that ranges between $8.1 - 5.8$; and Mazin, \cite{mazin2020}, (Cyan) reports a resolving power of $10$ at $808$ nm for hafnium (Hf) MKIDs. The experiments seem to be in good agreement with the trending of the modelled curve.
\begin{figure}[h!]
\begin{minipage}[b]{0.5\textwidth}
    \includegraphics[scale=0.23]{modelling/SNR-wavelength.png}
\end{minipage}
\begin{minipage}[b]{0.5\textwidth}
\includegraphics[scale=0.23]{modelling/P-energy.png}
\end{minipage}
\caption{Left: Signal to noise ratio $\frac{\Delta \alpha}{\alpha}$ as a function of the wavelength of the impinging photon. Right: Resolving power $\frac{E}{\Delta E}$ as a function of the energy of the photons that illuminate the resonator. The scatter plot represents experimentally measured points as collected from: Green - \cite{Guo}, Cyan - \cite{mazin2020}, Red - \cite{Szypryt_2017}.}
  \label{fig:DAA-lambda} 
\end{figure}{}


\section{Possible improvements} 
A final section is necessary to point out the results described in the previous pages and what technological improvements can be imagined might be relevant in future works. When it comes to the yield of an array, there is very little improvement that can be foreseen for superconductors such as $TiN_x$ for which it is known that $T_c$ homogeneity is very difficult. Other superconductors can exhibit a better uniformity, $TiN-Ti-TiN$ multilayers have not been tested thoroughly yet. The deposition of uniform and high quality thin films is well optimised for both $Ti$ and $TiN$. On a more technological stand point, an enhancement in the maximum frequency at which a low noise-temperature HEMT can operate, might allow the choice of sacrificing the close packing of an extra amount of resonators to improve the pixel yield. A further approach to maximise the yield would be the retuning of the colliding resonators through post-production processes such as trimming and DC-bias retuning \cite{DeLucia-multiplexing} (See chapter \ref{retuning}).\\
As previously discussed, the importance of the energy resolution of the detector is central and it is crucial for most application that it is as optimised as possible. The last few pages describe a model created $ad\,hoc$ to investigate the effects of several parameters on the energy resolution of an MKID: the noise temperature of the HEMT, which appeared to be the most significant contribution, the inhomogeneity in current density in the inductor of the resonator, the sampling frequency of the readout electronics and the  Fano noise that dominates the pair breaking process. The dominant contribution is provided by the HEMT, and very little can be done to minimise it. Of course a better HEMT has been in the community's wish list for several years now, and hopefully the parametric amplifiers currently under development \cite{Zobrist_2019} might be crucial for the further development of this technology. That said, Figure \ref{fig:HEMT_QQ} shows that a higher internal quality factor $Q_i$ can help improve the signal to noise ratio. Further improvement, on non dominant factors, is possible. New geometries can be investigated in order to maximise the current homogeneity, among these, a design with a large inductor could be interesting in order to minimise the effects of the current crowding at the right corners, whereas a tapered inductor could reduce the current density gradient. An in depth study of the physical properties of new materials, such as the multilayers and the Granular Aluminium, might produce interesting results in terms of quasi-particle life time, which would impact the contribution to the energy resolution given by the readout electronics. The Fano component issue is currently being addressed by the SRON group in the Netherlands,  by maximising the pair breaking efficiency $\eta$. In the case of semiconductors \cite{Fano_material} and gases \cite{fano_gas1}, the Fano factor has been observed to be material dependent. It might be worth investigating if there is a significant change in Fano noise across a broad variety of superconductors.
